CP-Router: An Uncertainty-Aware Router Between LLM and LRM

Recent advances in Large Reasoning Models (LRMs) have significantly improved long-chain reasoning capabilities over Large Language Models (LLMs). However, LRMs often produce unnecessarily lengthy outputs even for simple queries, leading to inefficiencies or even accuracy degradation compared to LLMs. To overcome this, we propose CP-Router, a training-free and model-agnostic routing framework that dynamically selects between an LLM and an LRM, demonstrated with multiple-choice question answering (MCQA) prompts. The routing decision is guided by the prediction uncertainty estimates derived via Conformal Prediction (CP), which provides rigorous coverage guarantees. To further refine the uncertainty differentiation across inputs, we introduce Full and Binary Entropy (FBE), a novel entropy-based criterion that adaptively selects the appropriate CP threshold. Experiments across diverse MCQA benchmarks, including mathematics, logical reasoning, and Chinese chemistry, demonstrate that CP-Router efficiently reduces token usage while maintaining or even improving accuracy compared to using LRM alone. We also extend CP-Router to diverse model pairings and open-ended QA, where it continues to demonstrate strong performance, validating its generality and robustness.

==> table/hypo_ensemble.tex <==
\begin{table*}[t]
\centering
\small
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule[0.5mm]
\multirow{2}{*}{\textbf{Strategy}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{ZH-EN}} & \multicolumn{2}{c}{\textbf{EN-ZH}} & \multirow{2}{*}{\textbf{Avg.}} \\ 
& & XCOMET & COMETKiwi & XCOMET & COMETKiwi & \\ \midrule
% \multirow{3}{*}{LLM} & Deepseek-R1 & 0.8388 & 0.7921 & 0.8302 & 0.7930 & 0.8135 \\
% & Deepseek-v3 & 0.8374 & 0.7909 & 0.8305 & 0.7943 & 0.8133 \\
% LLM ChooseBest& Gemini-2.0-Flash & 0.8325 & 0.7893 & 0.8098 & 0.7812 & 0.8032 \\
% \cdashlinelr{1-7}
\multirow{3}{*}{MBR} & BLEU & 0.8243 & 0.7842 & 0.8106 & 0.7768 & 0.7990 \\
& BERTScore & 0.8277 & 0.7874 & 0.8227 & 0.7837 & 0.8054 \\
& COMET & 0.8371 & 0.7932 & 0.8334 & 0.7949 & 0.8147 \\
% \cdashlinelr{1-7}
% \multirow{3}{*}{ORM} & ArmoRM-LLaMA3-8B-v0.1 & 0.8345 & 0.7915 & 0.8274 & 0.7951 & 0.8121 \\
% & Internlm2-7b-Reward & 0.8332 & 0.7920 & 0.8251 & 0.7959 & 0.8116 \\
% & Skywork-Reward-LLaMA-8B & 0.8296 & 0.7871 & 0.8251 & 0.7933 & 0.8088 \\
% & LLaMA-3B-Contrast & 0.7928 & 0.7663 & 0.7558 & 0.7359 & 0.7627 \\
% & LLaMA-3B-Token-DPO & 0.8039 & 0.7675 & 0.7654 & 0.7391 & 0.7690 \\
\cdashlinelr{1-7}
\multirow{3}{*}{Ranking} & Gemini-2.0-Flash & 0.8325 & 0.7893 & 0.8098 & 0.7812 & 0.8032 \\
& MT-PRM-Qwen2.5-3B & 0.8250 & 0.7866 & 0.8153 & 0.7841 & 0.8028 \\
& MT-PRM-LLaMA3.2-3B & 0.8282 & 0.7908 & 0.8225 & 0.7918 & 0.8083 \\
\bottomrule[0.5mm]
\end{tabular}
}
\caption{Automatic evaluation metrics for different ensembling strategies across WMT 23 ZH-EN and EN-ZH.}
\label{tab:ensemble} 
\end{table*}


==> table/main_tab.tex <==
\begin{table*}[t]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    \resizebox{2\columnwidth}{!}{
    \begin{tabular}{lcccccccccccc}
        \toprule[0.5mm]
        \multirow{2}{*}{Model} & \multicolumn{8}{c}{Sequence-level} & \multicolumn{4}{c}{Token-level} \\
        & \multicolumn{3}{c}{Prefixed} && \multicolumn{3}{c}{Arbitrary} && \multicolumn{3}{c}{Prefixed} \\
        \cline{2-4} \cline{6-8} \cline{10-12}
        \\
        & EN→XX & XX→EN & Avg. && EN→XX & XX→EN & Avg. && EN→XX & XX→EN & Avg. \\
        \midrule

        
        \multicolumn{4}{l}{\textcolor{gray}{\textit{Baselines}}}\\

        Skywork-Reward-LLaMA-3.1-8B & 0.857 & 0.773 & 0.815 && 0.768 & 0.743 & 0.756 && - & - & - \\
        MT-Ranker-base & 0.785 & 0.787 & 0.786 && 0.720 & 0.712 & 0.716 && - & - & - \\
        MT-Ranker-large & 0.847 & 0.873 & 0.860 && 0.750 & 0.805 & 0.778 && - & - & -\\
        \cdashlinelr{1-12}
        \multicolumn{4}{l}{\textcolor{gray}{\textit{PRMs}}}\\
        MT-PRM-LLaMA-3.2-3B & 0.777 & 0.775 & 0.776 && 0.675 & 0.660 & 0.668 && 0.542 &  0.615 & 0.578 \\
        MT-PRM-Qwen-2.5-3B & 0.867 & 0.858 & 0.863 && 0.622 & 0.633 & 0.628 && 0.637 & 0.685 & 0.660 \\

        \bottomrule[0.5mm]
    \end{tabular}
    }
    \caption{Accuracy results on RM-RewardBench. Skywork-Reward-LLaMA-3.1-8B is an advanced ORM for general domains, while MT-Ranker represents the SoTA non-metric reference-free translation quality estimation model.}
    \label{tab:main_results}
\end{table*}

==> table/prm_ablations.tex <==
\begin{table}[ht]
\centering

\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule[0.5mm]

 \textbf{Preference Pair Type}  & \textbf{Training Strategy} & \textbf{Avg.} \\\midrule
 % \raggedright{M-MAD-Consensus}  & {0.808} & {0.933} & {0.987} & {0.517} & {0.577} \\
 \raggedleft{Token-level} & {DPO} & {0.660}\\
 \raggedleft{Vanilla} & {DPO} & {0.574}\\
  \raggedleft{Token-level} & {KTO} & {0.644}\\
 \raggedleft{Vanilla} & {KTO} & {0.562} \\
\bottomrule[0.5mm]
\end{tabular}
}
\caption{Ablation study on the effect of training preference data and implicit reward training objectives. The backbone model is Qwen-2.5-3B-Instruct.}
\label{tab:ablation}
\end{table}
